Tools and Algorithms for SoC Communication Traces

In this paper, we study seven well-known trace analysis techniques both from the hardware and software domain and discuss their performance on communication-centric system-on-chip (SoC) traces. SoC traces are usually huge in size and concurrent in nature, therefore mining SoC traces poses additional challenges. We provide a hands-on discussion of the selected tools/algorithms in terms of the input, output, and analysis methods they employ. Hardware traces also varies in nature when observed in different level, this work can help developers/academicians to pick up the right techniques for their work. We take advantage of a synthetic trace generator to find the interestingness of the mined outcomes for each tool as well as we work with a realistic GEM5 set up to find the performance of these tools on more realistic SoC traces. Comprehensive analysis of the tool's performance and a benchmark trace dataset are also presented.

==> discussion.tex <==
\section{Discussions}
\label{sec:discussions}

In this section, we discuss a few observations and insights about \emph{FlowMiner} gained from experiments.

\smallskip
\noindent{\bf Mining Complex Patterns.} 
\emph{FlowMiner} can discover strong temporal relations among messages observed in a set of traces. It uses $100\%$ forward and backward confidence to mine assertions which hold over all traces.
%as we are interested in mining message flows implemented in SoC communication fabrics. 
The analysis of experimental results indicates that these two confidence measures, used together, allow flows with branching structures to be fully extracted from traces if those flows do not share common messages in their specifications. 

On the other hand, if multiple flows with branching structures and common messages are executed, then branches of those flows may not be completely mined.  One example includes two flows as shown in Figure~\ref{fig:ex} such that one is memory write for {\tt CPU\_0} ({\tt x=0}), while the other is memory write for {\tt CPU\_1} ({\tt x=1}).  These two flows share messages $m_5$ and $m_6$ for memory access.  The pattern $(m_3, m_4)$ may not be mined by \emph{FlowMiner} even though $(m_4,m_5,m_6, m_7)$ can be extracted.  This prevents the whole flow in Figure~\ref{fig:ex} from being found.  A typical technique for mining more patterns including those branching ones is to lower the confidence level.  Its drawback is the rapid increase in the total number of mined patterns, majority of which are invalid. %Additionally, finding a confidence level that balances the numbers of valid and invalid patterns can be tricky.  
In this work, we focus on developing the pattern chaining techniques instead of manipulating confidence levels.

\smallskip
\noindent{\bf Invalid Patterns.} Mining excessively large number of invalid patterns is a serious issue to limit specification mining in practical use.  The main reason for mining invalid patterns is the incorrect correlations among messages in traces. \emph{FlowMiner} uses address-based trace slicing and structural causality to exclude incorrect correlations from mining in a certain degree.  More such techniques would be beneficial to improving mining precision.    

%This bias is causing some patterns to be lost. Especially the scenario 4 in \ref{branching} is the type of flows that are out of scope of this tool. This is highly complex shared resources scenario. We call them branching in the flows. For example, two possible branches for this particular flow in Figure~\ref{fig:ex}: one from $t_1$ and another from $t_3$. $FlowMiner$ will search for assertions throughout the trace database. Here, $t_1$ can lead to $t_2$ or $t_10$. And $t_3$ can lead to $t_4$ or $t-9$. If $t_2$ has resulted from $t_1$ alone, then this branch ($t_1, t_2$) will have backward confidence of 100\%, thus will be extracted as an assertion. Similar resolution for $(t_1,t_10), (t_3, t_4)$ and $(t_3, t_9)$. On the other hand, if $t_2$ is also a branch of transition $t_x$, and $t_x$ has another branch $t_y$, then only forward and backward confidence are not enough to find these branches. Because $t_2$ is no more an assertion for transitions $t_1$ and $t_x$ in this extended scenario. To address such scenarios, we proposed mining for longer patterns(assertions). For example, if ($t_x,t_2$) is continually resulting to another set of transitions($t_a,t_b$), then ($t_x,t_2, t_a,t_b$) will constitute an assertion too, thus will be extracted.

%At this stage this tool is good at finding patterns that has many suffixes one prefix or vice versa. But if the SoC implements flows that bundles many suffixes, many prefixes ground truth together, $FlowMiner$ is not a good choice for them. 

\smallskip
\noindent{\bf Traces for Mining.} 
\emph{FlowMiner} can take any number of traces of different lengths provided as input for mining.  More patterns would be mined from longer traces as those traces may include more information about different flow executions.  The number of input traces can have an impact on mining precision as indicated in Section~\ref{sec:mining}.  Since temporal relations among messages extracted from traces are used approximate the causality relations, more input traces with diverse temporal orderings of flow executions can help to eliminate temporal relations that do not hold for all traces, thus reducing the number of invalid patterns to be mined.  

This work considers lossless traces, \ie~all messages of executed flows are captured in traces.  To deal with traces with missing messages,  we can lower the confidence levels.  The side effects of that approach are explained above.  Since \emph{FlowMiner} mines assertions, the patterns that involves missing messages cannot be mined.  In simulation environment, we think this may not be an issue.  A message can be missing due to 1) a design bug, or 2) incorrect instrumentation.  In the former case, a message may be missing only in a few spots in a trace.  On the other hand, a message will be always missing if the instrumentation for observation is set up incorrectly.  When the mining results are returned to the user for examination, the user can query the database of the mined patterns to filter out patterns that are deemed invalid, and to search for patterns that are expected to hold.  If an expected pattern is not included, it signals a problem in the simulation environment.  According to the above observation, the confidence levels of the sequence for a missing pattern can reveal the potential cause. If confidence levels of a missing pattern\footnote{A missing pattern refers to a sequence that is supposed to be pattern but is not mined due to missing messages.} are higher than 0, it is likely caused by a design bug.  Otherwise, incorrect instrumentation would be a more likely problem. 
 
%That means, if only a single transition out of millions traces misses a single event of a flow instance, this instance will not be treated as an assertion, thus won't be extracted.\\

% Should show runtime in results section.
%\textbf{Mining Time:} $FlowMiner$ is a rule based tool. It scans all the traces available. So mining time is proportional to number of traces to be scanned for assertions.



==> src-methodology-experiment.tex <==
\section{Methodology of Experiments}
\label{sec:methods}
Describe what and how to do it
\subsection{Evaluation Metrics}
\subsubsection{\#Binary Pattern}
\subsubsection{Execution Time}
\subsubsection{Precision}
\subsubsection{Recall}
\subsubsection{\#Patterns Mined}
\subsubsection{Longer Patterns}
